Incremental Versus Optimized Network Design

Even though the problem of network topology design is often studied as a "clean-slate" optimization, in practice most service-provider and enterprise networks are designed incrementally over time. This evolutionary process is driven by changes in the underlying parameters and constraints (the "environment") and it aims to minimize the modification cost after each change in the environment. In this paper, we first formulate the incremental design approach (in three variations), and compare that with the more traditional optimized design approach in which the objective is to minimize the total network cost. We evaluate the cost overhead and evolvability of incremental design under two network expansion models (random and gradual), comparing incremental and optimized networks in terms of cost, topological similarity, delay and robustness. We find that even though incremental design has some cost overhead, that overhead does not increase as the network grows. Also, it is less costly to evolve an existing network than to design it "from scratch" as long as the network expansion factor is less than a critical value.

==> Figures/robustness/Deg_BC_EVO.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,3960.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1960,1280){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1960,1647){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1960,2013){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1960,2380){\makebox(0,0)[r]{\strut{} 0.3}}%
      \put(1960,2746){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1960,3113){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1960,3479){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(2568,880){\makebox(0,0){\strut{} 2}}%
      \put(3304,880){\makebox(0,0){\strut{} 4}}%
      \put(4040,880){\makebox(0,0){\strut{} 6}}%
      \put(4775,880){\makebox(0,0){\strut{} 8}}%
      \put(5511,880){\makebox(0,0){\strut{} 10}}%
      \put(560,2379){\rotatebox{-270}{\makebox(0,0){\strut{}Betweenness Centrality}}}%
      \put(4039,280){\makebox(0,0){\strut{}Degree}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4136,3216){\makebox(0,0)[r]{\strut{}EVO}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figures/robustness/Deg_BC_EVO}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/robustness/Deg_BC_OPT.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,3960.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1960,1280){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1960,1647){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1960,2013){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1960,2380){\makebox(0,0)[r]{\strut{} 0.3}}%
      \put(1960,2746){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1960,3113){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1960,3479){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(2568,880){\makebox(0,0){\strut{} 2}}%
      \put(3304,880){\makebox(0,0){\strut{} 4}}%
      \put(4040,880){\makebox(0,0){\strut{} 6}}%
      \put(4775,880){\makebox(0,0){\strut{} 8}}%
      \put(5511,880){\makebox(0,0){\strut{} 10}}%
      \put(560,2379){\rotatebox{-270}{\makebox(0,0){\strut{}Betweenness Centrality}}}%
      \put(4039,280){\makebox(0,0){\strut{}Degree}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4136,3216){\makebox(0,0)[r]{\strut{}OPT}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figures/robustness/Deg_BC_OPT}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/robustness/cdf.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,3960.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1960,1280){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1960,1720){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1960,2160){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1960,2599){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1960,3039){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1960,3479){\makebox(0,0)[r]{\strut{} 1}}%
      \put(2200,880){\makebox(0,0){\strut{} 0}}%
      \put(2609,880){\makebox(0,0){\strut{} 0.05}}%
      \put(3018,880){\makebox(0,0){\strut{} 0.1}}%
      \put(3426,880){\makebox(0,0){\strut{} 0.15}}%
      \put(3835,880){\makebox(0,0){\strut{} 0.2}}%
      \put(4244,880){\makebox(0,0){\strut{} 0.25}}%
      \put(4653,880){\makebox(0,0){\strut{} 0.3}}%
      \put(5061,880){\makebox(0,0){\strut{} 0.35}}%
      \put(5470,880){\makebox(0,0){\strut{} 0.4}}%
      \put(5879,880){\makebox(0,0){\strut{} 0.45}}%
      \put(560,2379){\rotatebox{-270}{\makebox(0,0){\strut{}Emperical CDF}}}%
      \put(4039,280){\makebox(0,0){\strut{}Node Betweenness Centrality}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4136,3216){\makebox(0,0)[r]{\strut{}OPT}}%
      \csname LTb\endcsname%
      \put(4136,2816){\makebox(0,0)[r]{\strut{}EVO}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{cdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Makefile <==
TEXSRC=	*.tex

IMAGES= 

.SUFFIXES: .tex .dvi .ps .pdf .obj .eps

all: main.ps 

force:
	touch .rebuild
	make all

main.dvi: Makefile $(TEXSRC) $(IMAGES) .rebuild

.rebuild:
	touch .rebuild

.tex.dvi:
#	./src/process_images.pl ${IMAGES} $<
	latex \\nonstopmode \\input{$<}

.dvi.ps:
	#dvips -Ppdf -G0 -o $@ $<
	dvips -t letter -o $@ $<

.ps.pdf:
	ps2pdf12 $<

.obj.eps:
	@rm -f $@
	@TMPDIR=$${TMPDIR:-/tmp} tgif -print -eps $<


bib:
	latex main
	latex main
	latex main
	bibtex main
	bibtex main
	latex main
	latex main

clean:
	rm -f *.aux *.log *~ *.blg *.dvi

realclean: clean
	rm -f *.ps *.dvi *.pdf



==> conclusion.tex <==
We can now return to the questions that were asked in  
the introduction and summarize our main findings.
The following conclusions are supported by asymptotic 
scaling expressions for rings and by computational  
results in the case of mesh networks; it appears though
that the analytical expressions for rings also fit well the computational
results for the mesh networks we experimented with.\\
\noindent
1. We formulated the incremental network design process as
an optimization problem that aims to minimize the modification
cost relative to the previous network.
We also identified and compared certain expansion models 
(random versus gradual, and single-node versus multi-node) 
and three variations of the incremental
design process (Inventory, Ownership, Leasing). \\
2. Even though an evolved network has higher
cost than the corresponding optimized network, 
the cost overhead of the former does not increase as the network
grows, at least under single-node expansion.\\
3. In the case of mesh networks,
the incremental design process leads to networks 
with larger link density, higher performance in terms of the
average propagation delay across all primary paths, and improved
robustness in terms of a node betweenness centrality metric, compared
to optimized networks. 
These differences are more pronounced under random expansion.\\ 
4. Under single-node (random or gradual) expansion, 
it is less costly to follow the incremental design approach 
than to re-design the network from scratch. 
The evolvability under basic expansion approaches one as 
the network grows. \\
5. Under multi-node and random expansion, there is a critical value $\hat{\rho}$
of the expansion factor beyond which it is less costly to abandon the existing
network and re-design the network from scratch. It is not clear
whether this is ever the case under gradual expansion; our computational
experiments have never produced negative evolvability in that case. \\
6. The incremental and optimized design processes lead to significantly
different network topologies.
The evolved network has a more skewed degree distribution compared
to the optimized network, and it includes few nodes (hubs) with much 
higher degree and betweenness centrality than most other nodes.\\ 
7. The inventory overhead of the incremental design process does
not increase with time, and so the cumulative cost of the
inventory does not diverge relative to the cost of the evolved network.\\ 
8. Under gradual expansion, the evolvability is higher
and the cost overhead is lower than under random expansion.
The model of  gradual expansion represents a more ``evolution-friendly''
dynamic environment than random expansion.\\  
9. The Inventory option is a good compromise between cost overhead
and modification cost, compared to the Ownership and Leasing options.
If it is not possible to maintain an inventory, the Leasing option 
performs quite similar to the Inventory option.

In terms of future work, we believe that the previous questions can be 
studied more mathematically for specific regular or random network topologies,
deriving exact expressions. 
It would also be interesting to examine other dynamic environment models,
such as iterated multi-node expansion, models in which the traffic
loads and link capacities change with time as well, as well as more 
elaborate economic models that involve discounting or dynamic costs.
It would also be interesting to see this quantitative framework
and comparisons between evolved and optimized designs applied in other   
problems and technological domains.

